Expanding the Action Space of LLMs to Reason Beyond Language

Large Language Models (LLMs) are powerful reasoners in natural language, but their actions are typically confined to outputting vocabulary tokens. As a result, interactions with external environments -- such as symbolic operators or simulators -- must be expressed through text in predefined formats, parsed, and routed to external interfaces. This overloads the model's language with both reasoning and control duties, and requires a hand-crafted parser, external to the LLM. To address this, we decouple environment interactions from language by internalizing them in an Expanded Action space (ExpA), beyond the vocabulary. The model starts reasoning in the default language environment, but may trigger routing actions and switch to an external environment at any time. From there, the model can only invoke environment-specific actions, receive feedback from the environment, and potentially route back to language as a result. To promote effective exploration of the expanded action space and new environments, we introduce ExpA Reinforcement Learning (EARL) with counterfactual policy optimization. On tasks requiring multi-turn interactions and contingent planning, EARL outperforms strong baselines with vocabulary-constrained actions. It performs robustly across calculator-based multi-task learning and, in the partially observed sorting problem, achieves perfect Sort-4 accuracy while self-discovering an efficient algorithm competitive with classical designs.

==> resources/figures/fig_tree_reference.tex <==

\definecolor{mygreen}{RGB}{0,150,80}
\definecolor{mycolor_0-1}{RGB}{150, 150, 255}
\definecolor{mycolor_0}{RGB}{248, 248, 255}
\definecolor{mycolor_1-1}{RGB}{0, 180, 180}
\definecolor{mycolor_1}{RGB}{243, 255, 255}
\definecolor{mycolor_2-1}{RGB}{238, 181, 0}
\definecolor{mycolor_2}{RGB}{255, 253, 247}
\definecolor{mycolor_3-1}{RGB}{0, 140, 215}
\definecolor{mycolor_3}{RGB}{230, 249, 251}
\definecolor{mycolor_4-1}{RGB}{40, 160, 37}
\definecolor{mycolor_4}{RGB}{238, 252, 238}
\definecolor{mycolor_5-1}{RGB}{33, 94, 153}
\definecolor{mycolor_5}{RGB}{237, 244, 249}
\definecolor{mycolor_6-1}{RGB}{215, 109, 204}
\definecolor{mycolor_6}{RGB}{252, 242, 252}
\definecolor{mycolor_7-1}{RGB}{77, 148, 216}
\definecolor{mycolor_7}{RGB}{236, 239, 255}
\definecolor{mycolor_8-1}{RGB}{30, 40, 50}
\definecolor{mycolor_8}{RGB}{230, 245, 255}
\definecolor{mycolor_tab-1}{RGB}{255, 255, 255}
\definecolor{mycolor_tab-2}{RGB}{234, 248, 253}
\definecolor{darkcyan}{RGB}{0, 139, 139}

\tikzstyle{leaf}=[draw=hiddendraw,
    rounded corners, minimum height=1em,
    fill=mygreen!40,text opacity=1, 
    fill opacity=.5,  text=black,align=left,font=\scriptsize,
    inner xsep=3pt,
    inner ysep=1pt,
    ]
\tikzstyle{middle}=[draw=hiddendraw,
    rounded corners, minimum height=1em,
    fill=output-white!40,text opacity=1, 
    fill opacity=.5,  text=black,align=center,font=\scriptsize,
    inner xsep=7pt,
    inner ysep=1pt,
    ]



\begin{forest}
    for tree={
        forked edges,
        grow=east,
        reversed=true,
        anchor=base west,
        parent anchor=east,
        child anchor=west,
        base=middle,
        font=\scriptsize,
        rectangle,
        line width=0.1pt,
        draw = black!40,
        rounded corners=2pt,
        align=left,
        minimum width=2em, 
        s sep=6pt, 
        l sep=8pt,
        inner xsep = 2pt,
        inner ysep = 2pt,
        edge path={
          \noexpand\path [draw, \forestoption{edge}]
          (!u.parent anchor) -- ++(1.5mm,0) |- (.child anchor) \forestoption{edge label};},
        ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
        font=\linespread{1}\selectfont,
    },
    where level=1{font=\footnotesize,fill=blue!0}{},
    where level=2{font=\footnotesize,fill=pink!0}{},
    where level=3{font=\footnotesize,fill=green!0}{},
    where level=4{font=\footnotesize,fill=mygreen!5}{},
    where level=5{font=\footnotesize,fill=mygreen!5}{},
    where level=6{font=\footnotesize,fill=mygreen!5}{},
    [{LLM Implicit Reasoning}, ver, color=mycolor_0-1, fill=mycolor_0, text=black, font=\footnotesize, text width=70em, text centered, inner ysep=8pt
        [Introduction (\S\ref{sec:Introduction}), color=mycolor_1-1, fill=mycolor_1, text=black, inner xsep=6pt, inner ysep=6pt, text width=7.9em
        ]
        [Preliminaries (\S\ref{sec:Preliminaries}), color=mycolor_2-1, fill=mycolor_2, text=black, inner xsep=6pt, inner ysep=6pt, text width=7.9em
            [General LLM Reasoning \\(\S\ref{sec:preliminary_general-LLM-reasoning}), color=mycolor_2-1, fill=mycolor_2, text=black, inner xsep=6pt, inner ysep=2.5pt, text width=11em
            ]
            [LLM Explicit Reasoning \\(\S\ref{sec:preliminary_explicit}), color=mycolor_2-1, fill=mycolor_2, text=black, inner xsep=6pt, inner ysep=2.5pt, text width=11em
            ]
            [LLM Implicit Reasoning \\(\S\ref{sec:preliminary_implicit}), color=mycolor_2-1, fill=mycolor_2, text=black, inner xsep=6pt, inner ysep=2.5pt, text width=11em
            ]
            [Explicit vs Implicit Reasoning \\(\S\ref{sec:preliminary_explicit-vs-implicit}), color=mycolor_2-1, fill=mycolor_2, text=black, inner xsep=6pt, inner ysep=2.5pt, text width=11em
            ]
        ]
        [{Technical Paradigms (\S\ref{sec:techinical-paradigm})}, color=mycolor_3-1, fill=mycolor_3, text=black, inner xsep=6pt, inner ysep=6pt, inner ysep=6pt, text width=10em
            [{Latent Optimization \\(\S\ref{sec:technical-paradigm_latent-optimization})}, color=mycolor_3-1, fill=mycolor_3, text=black, inner xsep=6pt, inner ysep=4pt, text width=9em
                [{Token-Level \\(\S\ref{sec:technical-paradigm_latent-optimization_token})}, color=mycolor_3-1, fill=mycolor_3, text=black, inner xsep=6pt, inner ysep=4pt, text width=7em
                    [{
                        CoCoMix~\citep{2025_arXiv_CoCoMix_LLM-Pretraining-with-Continuous-Concepts},
                        Latent Token~\citep{2025_arXiv_Latent-Token_Enhancing-Latent-Computation-in-Transformers-with-Latent-Tokens}, \\[0.3em]
                        LPC~\citep{2025_ICML_LPC_Latent-Preference-Coding-Aligning-Large-Language-Models-via-Discrete-Latent-Codes},
                        Token Assorted~\citep{2025_ICML_Token-Assorted_Token-Assorted-Mixing-Latent-and-Text-Tokens-for-Improved-Language-Model-Reasoning}\\
                    }, color=mycolor_3-1, fill=mycolor_3, text=black, inner xsep=6pt, inner ysep=4pt, text width=26em
                    ]
                ]
                [{Trajectory-Level \\(\S\ref{sec:technical-paradigm_latent-optimization_trajectory})}, color=mycolor_3-1, fill=mycolor_3, text=black, inner xsep=6pt, inner ysep=4pt, text width=7em
                    [{Semantic Anchoring \\(\S\ref{sec:technical-paradigm_latent-optimization_trajectory_sematic-anchoring}\textcolor{blue}{(a)})}, color=mycolor_3-1, fill=mycolor_3, text=black, inner xsep=6pt, inner ysep=4pt, text width=9.7em
                        [{
                            CCoT~\citep{2024_arXiv_CCoT_Compressed-Chain-of-Thought-Efficient-Reasoning-through-Dense-Representations},\\[0.3em]
                            HCoT~\citep{2024_arXiv_HCoT_Expediting-and-Elevating-Large-Language-Model-Reasoning-via-Hidden-Chain-of-thought-Decoding},\\[0.3em]
                            CODI~\citep{2025_arXiv_CODI_CODI=Compressing-Chain-of-thought-into-Continuous-Space-via-Self-Distillation},\\[0.3em]
                            SynAdapt~\citep{2025_arXiv_SynAdapt_SynAdapt=Learning-Adaptive-Reasoning-in-Large-Language-Models-via-Synthetic-Continuous-Chain-of-thought}
                        }, color=mycolor_3-1, fill=mycolor_3, text=black, inner xsep=6pt, inner ysep=4pt, text width=14.3em
                        ]
                    ]
                    [{Adaptive Efficiency \\(\S\ref{sec:technical-paradigm_latent-optimization_trajectory_adaptive}\textcolor{blue}{(b)})}, color=mycolor_3-1, fill=mycolor_3, text=black, inner xsep=6pt, inner ysep=4pt, text width=9.7em
                        [{
                            LightThinker~\citep{2025_arXiv_LightThinker_LightThinker=Thinking-Step-by-step-Compression},\\[0.3em]
                            CoT-Valve~\citep{2025_arXiv_CoT-Valve_CoT-Valve=Length-Compressible-Chain-of-thought-Tuning},\\[0.3em]
                            CoLaR~\citep{2025_arXiv_CoLaR_Think-Silently-Think-Fast=Dynamic-Latent-Compression-of-LLM-Reasoning-Chains}
                        }, color=mycolor_3-1, fill=mycolor_3, text=black, inner xsep=6pt, inner ysep=4pt, text width=14.3em
                        ]
                    ]
                    [{Progressive Refinement \\(\S\ref{sec:technical-paradigm_latent-optimization_trajectory_progressive}\textcolor{blue}{(c)})}, color=mycolor_3-1, fill=mycolor_3, text=black, inner xsep=6pt, inner ysep=4pt, text width=9.7em
                        [{
                            ICoT-SI~\citep{2024_arXiv_ICoT-SI_From-Explicit-CoT-to-Implicit-CoT=Learning-to-Internalize-CoT-Step-by-Step},\\[0.3em]
                            Coconut~\citep{2024_arXiv_Coconut-ProsQA-dataset_Training-Large-Language-Models-to-Reason-in-a-Continuous-Latent-Space},\\[0.3em]
                            Heima~\citep{2025_arXiv_Heima_Efficient-Reasoning-with-Hidden-Thinking},\\[0.3em]
                            PonderingLM \citep{2025_arXiv_PonderingLM_Pretraining-Language-Models-to-Ponder-in-Continuous-Space},\\[0.3em]
                            BoLT~\citep{2025_arXiv_BoLT_Reasoning-to-Learn-from-Latent-Thoughts}
                        }, color=mycolor_3-1, fill=mycolor_3, text=black, inner xsep=6pt, inner ysep=4pt, text width=14.3em
                        ]
                    ]
                    [{Exploratory Diversification \\(\S\ref{sec:technical-paradigm_latent-optimization_trajectory_exploratory}\textcolor{blue}{(d)})}, color=mycolor_3-1, fill=mycolor_3, text=black, inner xsep=6pt, inner ysep=4pt, text width=9.7em
                        [{
                            LaTRO~\citep{2024_arXiv_LaTRO_Language-Models-are-Hidden-Reasoners=Unlocking-Latent-Reasoning-Capabilities-via-Self-rewarding},\\[0.3em]
                            Soft Thinking~\citep{2025_arXiv_Soft-Thinking_Soft-Thinking=Unlocking-the-Reasoning-Potential-of-LLMs-in-Continuous-Concept-Space},\\[0.3em]
                            SoftCoT~\citep{2025_arXiv_SoftCoT_SoftCoT=Soft-Chain-of-thought-For-Efficient-Reasoning-with-LLMs},\\[0.3em]
                            SoftCoT++~\citep{2025_arXiv_SoftCoT++_SoftCoT++=Test-Time-Scaling-with-Soft-Chain-of-Thought-Reasoning},\\[0.3em]
                            COT2~\citep{2025_arXiv_COT2_Continuous-Chain-of-Thougth-Enables-Parallel-Exploration-and-Reasoning}
                        }, color=mycolor_3-1, fill=mycolor_3, text=black, inner xsep=6pt, inner ysep=4pt, text width=14.3em
                        ]
                    ]
                ]
                [{Internal-State-Level \\(\S\ref{sec:technical-paradigm_latent-optimization_internal-state})}, color=mycolor_3-1, fill=mycolor_3, text=black, inner xsep=6pt, inner ysep=4pt, text width=7em
                    [{
                        ICoT-KD~\citep{2023_arXiv_ICoT-KD_Implicit-Chain-of-Thought-Reasoning-via-Knowledge-Distillation},
                        System2 Distillation~\citep{2024_NeurIPS-Workshop_Distilling-System-2-into-System-1},\\[0.3em]
                        LTMs~\citep{2025_ICML_LTMs_Scalable-Language-Models-with-Posterior-Inference-of-Latent-Thought-Vectors},
                        System-1.5 Reasoning~\citep{2025_arXiv_System-1.5-Reasoning_System-1.5-Reasoning=Traversal-in-Language-and-Latent-Spaces-with-Dynamic-Shortcuts},  \\[0.3em]
                        Beyond Words~\citep{2025_arXiv_Beyond-Words_Beyond-Words=A-Latent-Memory-Approach-to-Internal-Reasoning-in-LLMs}, 
                        ReaRec~\citep{2025_arXiv_ReaRec_Think-before-Recommend=Unleashing-the-Latent-Reasoning-Power-for-Sequential-Recommendation}, \\[0.3em]
                        HRPO~\citep{2025_arXiv_HRPO_Hybrid-Latent-Reasoning-via-Reinforcement-Learning}
                        }, color=mycolor_3-1, fill=mycolor_3, text=black, inner xsep=6pt, inner ysep=4pt, text width=26em
                    ]
                ]
            ]
            [{Signal-Guided Control \\ (\S\ref{sec:technical-paradigm_control})}, color=mycolor_3-1, fill=mycolor_3, text=black, inner xsep=6pt, inner ysep=4pt, text width=9em
                [{Single‑Type Signal \\(\S\ref{sec:technical-paradigm_control_single-type-signal})}, color=mycolor_3-1, fill=mycolor_3, text=black, inner xsep=6pt, inner ysep=4pt, text width=7em
                    [{
                        Thinking Tokens~\citep{2024_arXiv_thinking-tokens_Thinking-Tokens-for-Language-Modeling}, \\[0.3em]
                        Pause Tokens~\citep{2024_ICLR_pause-tokens_Think-Before-You-Speak=Training-Language-Models-with-Pause-Tokens},
                        Filler Tokens~\citep{2024_CoLM_filler-tokens_Let's-Think-Dot-by-Dot=Hidden-Computation-in-Transformer-Language-Models}, \\[0.3em]
                        Planning Tokens~\citep{2024_COLM_planning-tokens_Guiding-Language-Model-Reasoning-with-Planning-Tokens}, \\[0.3em]
                        Quiet-STaR~\citep{2024_COLM_Quiet-STaR_Quiet-STaR=Language-Models-Can-Teach-Themselves-to-Think-Before-Speaking}, 
                        LatentSeek~\citep{2025_arXiv_LatentSeek_Seek-in-the-dark=Reasoning-via-test-time-instance-level-policy-gradient-in-latent-space}, \\[0.3em]
                        DIT~\citep{2025_arXiv_2025_ACL_DIT_Learning-to-Insert-PAUSE-Tokens-for-Better-Reasoning}
                    }, color=mycolor_3-1, fill=mycolor_3, text=black, inner xsep=6pt, inner ysep=4pt, text width=26em
                    ]
                ]
                [{Multi‑Type Signal \\ (\S\ref{sec:technical-paradigm_control_multi-type-signal})}, color=mycolor_3-1, fill=mycolor_3, text=black, inner xsep=6pt, inner ysep=4pt, text width=7em
                    [{
                        Memory \& Reasoning~\citep{2024_arXiv_2025_ACL_Memory-Reasoning_Disentangling-Memory-and-Reasoning-Ability-in-Large-Language-Models}, 
                        Thinkless~\citep{2025_arxiv_Thinkless_Thinkless=LLM-Learns-When-to-Think}
                    }, color=mycolor_3-1, fill=mycolor_3, text=black, inner xsep=6pt, inner ysep=4pt, text width=26em
                    ]
                ]
            ]
            [{Layer‑Recurrent Execution (\S\ref{sec:technical-paradigm_recurrent})}, color=mycolor_3-1, fill=mycolor_3, text=black, inner xsep=6pt, inner ysep=4pt, text width=18em
                [{
                    ITT~\citep{2025_arXiv_ITT_Inner-Thinking-Transformer=Leveraging-Dynamic-Depth-Scaling-to-Foster-Adaptive-Internal-Thinking},
                    looped Transformer~\citep{2025_arXiv_2025_ICLR_looped-Transformer_Reasoning-with-Latent-Thoughts=On-the-Power-of-Looped-Transformers} \\[0.3em]
                    CoTFormer~\citep{2025_ICLR_CoTFormer_CoTFormer=A-Chain-of-Thought-Driven-Architecture-with-Budged-Adaptive-Computation-Cost-at-Inference}, 
                    Huginn~\citep{2025_arXiv_Huginn_Scaling-up-Test-Time-Compute-with-Latent-Reasoning=A-Recurrent-Depth-Approach}, \\[0.3em]
                    RELAY~\citep{2025_arXiv_RELAY_Enhancing-Auto-regressive-Chain-of-Thought-through-Loop-Aligned-Reasoning}
                }, color=mycolor_3-1, fill=mycolor_3, text=black, inner xsep=6pt, inner ysep=4pt, text width=26em
                ]
            ]
        ]
        [{Mechanistic and Behavioral \\Evidence (\S\ref{sec:evidence})}, color=mycolor_4-1, fill=mycolor_4, text=black, inner xsep=6pt, inner ysep=6pt, text width=10em,
            [Layer-wise Structural Evidence (\S\ref{sec:evidence_layer-wise-structural}), color=mycolor_4-1, fill=mycolor_4, text=black, inner xsep=6pt, inner ysep=4pt, text width=18em
                [{
                    Jump to Conclusions~\citep{2024_LREC-COLING_Jump-to-Conclusions=Short-Cutting-Transformers-with-Linear-Transformations}, \\[0.3em]
                    LM Implicit Reasoning~\citep{2025_arXiv_LM-Implicit-Reasoning_Implicit-Reasoning-in-Transformers-is-Reasoning-through-Shortcuts}, \\[0.3em]
                    Internal Chain-of-Thought~\citep{2025_arXiv_Internal-Chain-of-thought=Empirical-Evidence-for-Layer-wise-Subtask-Scheduling-in-LLMs}, \\[0.3em]
                    Reasoning by Superposition~\citep{2025_arXiv_Reasoning-by-Superposition=A-Theoretical-Perspective-on-Chain-of-Continuous-Thought}, \\[0.3em]
                    To CoT or To Loop~\citep{2025_arXiv_To-CoT-or-to-Loop=A-Formal-Comparison-Between-Chain-of-thought-and-Looped-Transformers}
                }, color=mycolor_4-1, fill=mycolor_4, text=black, inner xsep=6pt, inner ysep=4pt, inner ysep=4pt, text width=26em
                ]
            ]
            [Behavioral Signatures (\S\ref{sec:evidence_behavioral-signatures}), color=mycolor_4-1, fill=mycolor_4, text=black, inner xsep=6pt, inner ysep=4pt, text width=18em
                [{
                    Grokked Transformer \citep{2024_arXiv_Grokked-Transformer_Grokked-Transformers-are-Implicit-Reasoners=A-Mechanistic-Journey-to-the-Edge-of-Generalization}, \\
                    Latent Multi-Hop Reasoning~\citep{2024_ACL_latent-multi-hop-reasoning_Do-Large-Language-Models-Latently-Perform-Multi-hop-Reasoning}, \\
                    Step-skipping~\citep{2024_NeurIPS_step-skipping_Can-Language-Models-Learn-to-Skip-Steps}, \\
                    Beyond Chains of Thought \citep{2025_arXiv_Beyond-Chains-of-Thought=Benchmarking-Latent-Space-Reasoning-Abilities-in-Large-Language-Models}
                }, color=mycolor_4-1, fill=mycolor_4, text=black, inner xsep=6pt, inner ysep=4pt, text width=26em
                ]
            ]
            [Representation-Based Analysis (\S\ref{sec:evidence_representation-based}), color=mycolor_4-1, fill=mycolor_4, text=black, inner xsep=6pt, inner ysep=4pt, text width=18em
                [{
                    MechanisticProbe \citep{2023_EMNLP_MechanisticProbe_Towards-a-Mechanistic-Interpretation-of-Multi-Step-Reasoning-Capabilities-of-Language-Models}, 
                    TTT~\citep{2024_arXiv_TTT_Think-to-Talk-or-Talk-to-Think=When-LLMs-Come-Up-with-an-Answer-in-Multi-Step-Arithmetic-Reasoning}, \\
                    \citet{2024_arXiv_Do-LLMs-Really-Think-Step-by-Step-in-Implicit-Reasoning}, 
                    Distributional Reasoing~\citep{2024_arXiv_Distributional-Reasoning_Distributional-Reasoning-in-LLMs=Parallel-Reasoning-Processes-in-Multi-hop-Reasoning}, \\ 
                    Steering Vector Intervention~\citep{2025_ICLR-Workshop_steering-vector-intervention_Uncovering-Latent-Chain-of-Thought-Vectors-in-Large-Language-Models},   \\
                    Backward Chaining Circuits~\citep{2024_ACL_backward-chaining-circuits_A-Mechanistic-Analysis-of-a-Transformer-Trained-on-a-Symbolic-Multi-Step-Reasoning-Task}, \\[0.3em]
                    CoE~\citep{2024_arXiv_2025_ICLR_CoE_Latent-Space-Chain-of-Embedding-Enables-Output-free-LLM-Self-Evaluation}
                }, color=mycolor_4-1, fill=mycolor_4, text=black, inner xsep=6pt, inner ysep=4pt, text width=26em
                ]
            ]
        ]
        [{Evaluation and \\Benchmarking (\S\ref{sec:Evaluation-and-Benchmark})}, color=mycolor_5-1, fill=mycolor_5, text=black, inner xsep=6pt, inner ysep=6pt, text width=10em   
            [Metrics (\S\ref{sec:evaluation-and-benchmark_metrics}), color=mycolor_5-1, fill=mycolor_5, text=black, inner xsep=6pt, inner ysep=4pt, text width=18em   
            ]
            [Benchmarks (\S\ref{sec:evaluation-and-benchmark_benchmarks}), color=mycolor_5-1, fill=mycolor_5, text=black, inner xsep=6pt, inner ysep=4pt, text width=18em   
                [General Knowledge and Commonsense Reasoning (\S\ref{sec:benchmark_commonsenese}), color=mycolor_5-1, fill=mycolor_5, text=black, inner xsep=6pt, inner ysep=2.5pt, text width=26em   
                ]
                [Mathematical Reasoning and Programming (\S\ref{sec:benchmark_mathematical-and-programming}), color=mycolor_5-1, fill=mycolor_5, text=black, inner xsep=6pt, inner ysep=2.5pt, text width=26em   
                ]
                [Language Modeling and Reading Comprehension (\S\ref{sec:benchmark_language-modeling-and-reading-comprehension}), color=mycolor_5-1, fill=mycolor_5, text=black, inner xsep=6pt, inner ysep=2.5pt, text width=26em   
                ]
                [Complex Multi-Hop and Multidisciplinary QA (\S\ref{sec:benchmark_multi-hop-and-multidisciplinary-QA}), color=mycolor_5-1, fill=mycolor_5, text=black, inner xsep=6pt, inner ysep=2.5pt, text width=26em   
                ]
                [Multi-modal Reasoning (\S\ref{sec:benchmark_multi-modal}), color=mycolor_5-1, fill=mycolor_5, text=black, inner xsep=6pt, inner ysep=2.5pt, text width=26em   
                ]
            ]
        ]
        [{Challenges and \\Limitations (\S\ref{sec:Challenges-and-Future-Directions})}, color=mycolor_6-1, fill=mycolor_6, text=black, inner xsep=6pt, inner ysep=6pt, text width=10em
            [{
                $\circ$ Limited Interpretability and Latent Opacity
                \hspace{6.35em} $\circ$ Limited Control and Reliability \\
                $\circ$ Performance Gap Compared to Explicit Reasoning
                \hspace{3.45em} $\circ$ Lack of Standardized Evaluation \\
                $\circ$ Architecture and Generalization Constraints
                \hspace{6.26em} $\circ$ Dependence on Explicit Supervision
                }, color=mycolor_6-1, fill=mycolor_6, text=black, inner xsep=6pt, inner ysep=6pt, text width=46em
            ]
        ]        
        [Conclusion (\S\ref{sec:Conclusion}), color=mycolor_7-1, fill=mycolor_7, text=black, inner xsep=6pt, inner ysep=6pt, text width=10em
        ]
    ]
\end{forest}

==> resources/figures/related_work_fig_example.tex <==

\definecolor{mygreen}{RGB}{0,150,80}
\definecolor{mycolor_0-1}{RGB}{150, 150, 255}
\definecolor{mycolor_0}{RGB}{248, 248, 255}
\definecolor{mycolor_1-1}{RGB}{0, 180, 180}
\definecolor{mycolor_1}{RGB}{243, 255, 255}
\definecolor{mycolor_2-1}{RGB}{238, 181, 0}
\definecolor{mycolor_2}{RGB}{255, 253, 247}
\definecolor{mycolor_3-1}{RGB}{0, 140, 215}
\definecolor{mycolor_3}{RGB}{230, 249, 251}
\definecolor{mycolor_4-1}{RGB}{40, 160, 37}
\definecolor{mycolor_4}{RGB}{238, 252, 238}
\definecolor{mycolor_5-1}{RGB}{33, 94, 153}
\definecolor{mycolor_5}{RGB}{237, 244, 249}
\definecolor{mycolor_6-1}{RGB}{215, 109, 204}
\definecolor{mycolor_6}{RGB}{252, 242, 252}
\definecolor{mycolor_7-1}{RGB}{77, 148, 216}
\definecolor{mycolor_7}{RGB}{236, 239, 255}
\definecolor{mycolor_8-1}{RGB}{30, 40, 50}
\definecolor{mycolor_8}{RGB}{230, 245, 255}
\definecolor{mycolor_tab-1}{RGB}{255, 255, 255}
\definecolor{mycolor_tab-2}{RGB}{234, 248, 253}
\definecolor{darkcyan}{RGB}{0, 139, 139}

\tikzstyle{leaf}=[draw=hiddendraw,
    rounded corners, minimum height=1em,
    fill=mygreen!40,text opacity=1, 
    fill opacity=.5,  text=black,align=left,font=\normalsize,
    inner xsep=3pt,
    inner ysep=1pt,
    ]
\tikzstyle{middle}=[draw=hiddendraw,
    rounded corners, minimum height=1em,
    fill=output-white!40,text opacity=1, 
    fill opacity=.5,  text=black,align=center,font=\normalsize,
    inner xsep=7pt,
    inner ysep=1pt,
    ]



\begin{forest}
    for tree={
        forked edges,
        grow=east,
        reversed=true,
        anchor=base west,
        parent anchor=east,
        child anchor=west,
        base=middle,
        font=\scriptsize,
        rectangle,
        line width=0.1pt,
        draw = black!40,
        rounded corners=2pt,
        align=left,
        minimum width=2em, 
        s sep=6pt, 
        l sep=8pt,
        inner xsep = 2pt,
        inner ysep = 2pt,
        edge path={
          \noexpand\path [draw, \forestoption{edge}]
          (!u.parent anchor) -- ++(1.5mm,0) |- (.child anchor) \forestoption{edge label};},
        ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
        font=\linespread{1}\selectfont,
    },
    where level=1{font=\normalsize,fill=blue!0}{},
    where level=2{font=\normalsize,fill=pink!0}{},
    where level=3{font=\normalsize,fill=green!0}{},
    where level=4{font=\normalsize,fill=mygreen!5}{},
    where level=5{font=\normalsize,fill=mygreen!5}{},
    where level=6{font=\normalsize,fill=mygreen!5}{},
    [{LLM Action Space Expension}, ver, color=mycolor_0-1, fill=mycolor_0, text=black, font=\large, text width=40em, text centered, inner ysep=8pt
        [{Architecture A (\S\ref{sec:evidence})}, color=mycolor_4-1, fill=mycolor_4, text=black, inner xsep=6pt, inner ysep=6pt, text width=10em,
            [Partially Observed (\S\ref{sec:evidence_layer-wise-structural}), color=mycolor_4-1, fill=mycolor_4, text=black, inner xsep=6pt, inner ysep=4pt, text width=18em
                [{
                    Jump to Conclusions~\citep{2024_LREC-COLING_Jump-to-Conclusions=Short-Cutting-Transformers-with-Linear-Transformations}, \\[0.3em]
                    LM Implicit Reasoning~\citep{2025_arXiv_LM-Implicit-Reasoning_Implicit-Reasoning-in-Transformers-is-Reasoning-through-Shortcuts}, \\[0.3em]
                    Internal Chain-of-Thought~\citep{2025_arXiv_Internal-Chain-of-thought=Empirical-Evidence-for-Layer-wise-Subtask-Scheduling-in-LLMs}, \\[0.3em]
                    Reasoning by Superposition~\citep{2025_arXiv_Reasoning-by-Superposition=A-Theoretical-Perspective-on-Chain-of-Continuous-Thought}, \\[0.3em]
                    To CoT or To Loop~\citep{2025_arXiv_To-CoT-or-to-Loop=A-Formal-Comparison-Between-Chain-of-thought-and-Looped-Transformers}
                }, color=mycolor_4-1, fill=mycolor_4, text=black, inner xsep=6pt, inner ysep=4pt, inner ysep=4pt, text width=26em
                ]
            ]
            [Fully Observed (\S\ref{sec:evidence_behavioral-signatures}), color=mycolor_4-1, fill=mycolor_4, text=black, inner xsep=6pt, inner ysep=4pt, text width=18em
                [{
                    Grokked Transformer \citep{2024_arXiv_Grokked-Transformer_Grokked-Transformers-are-Implicit-Reasoners=A-Mechanistic-Journey-to-the-Edge-of-Generalization}, \\
                    Latent Multi-Hop Reasoning~\citep{2024_ACL_latent-multi-hop-reasoning_Do-Large-Language-Models-Latently-Perform-Multi-hop-Reasoning}, \\
                    Step-skipping~\citep{2024_NeurIPS_step-skipping_Can-Language-Models-Learn-to-Skip-Steps}, \\
                    Beyond Chains of Thought \citep{2025_arXiv_Beyond-Chains-of-Thought=Benchmarking-Latent-Space-Reasoning-Abilities-in-Large-Language-Models}
                }, color=mycolor_4-1, fill=mycolor_4, text=black, inner xsep=6pt, inner ysep=4pt, text width=26em
                ]
            ]
        ]
        [{Architecture C (\S\ref{sec:Evaluation-and-Benchmark})}, color=mycolor_5-1, fill=mycolor_5, text=black, inner xsep=6pt, inner ysep=6pt, text width=10em   
            [Partially Observed (\S\ref{sec:evaluation-and-benchmark_metrics}), color=mycolor_5-1, fill=mycolor_5, text=black, inner xsep=6pt, inner ysep=4pt, text width=18em   
            ]
            [Fully Observed (\S\ref{sec:evaluation-and-benchmark_benchmarks}), color=mycolor_5-1, fill=mycolor_5, text=black, inner xsep=6pt, inner ysep=4pt, text width=18em   
                [General Knowledge and Commonsense Reasoning (\S\ref{sec:benchmark_commonsenese}), color=mycolor_5-1, fill=mycolor_5, text=black, inner xsep=6pt, inner ysep=2.5pt, text width=26em   
                ]
                [Mathematical Reasoning and Programming (\S\ref{sec:benchmark_mathematical-and-programming}), color=mycolor_5-1, fill=mycolor_5, text=black, inner xsep=6pt, inner ysep=2.5pt, text width=26em   
                ]
                [Language Modeling and Reading Comprehension (\S\ref{sec:benchmark_language-modeling-and-reading-comprehension}), color=mycolor_5-1, fill=mycolor_5, text=black, inner xsep=6pt, inner ysep=2.5pt, text width=26em   
                ]
                [Complex Multi-Hop and Multidisciplinary QA (\S\ref{sec:benchmark_multi-hop-and-multidisciplinary-QA}), color=mycolor_5-1, fill=mycolor_5, text=black, inner xsep=6pt, inner ysep=2.5pt, text width=26em   
                ]
                [Multi-modal Reasoning (\S\ref{sec:benchmark_multi-modal}), color=mycolor_5-1, fill=mycolor_5, text=black, inner xsep=6pt, inner ysep=2.5pt, text width=26em   
                ]
            ]
        ]        
    ]
\end{forest}

==> resources/figures/token_length_analysis.tex <==
\begin{figure}[!t]
  \begin{subfigure}[b]{0.44\textwidth}
    \includegraphics[width=\textwidth]{resources/figures/cumulative_fraction_plot.pdf}
    \caption{}
    \label{token_len:f1}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{resources/figures/toekn_analysis.pdf}
    \caption{}
    \label{token_len:f2}
  \end{subfigure}
  \caption{\ws{replace (a) with countdown analysis}(a): cumulative fraction of predictions by number
of tokens in the reasoning output, grouped by whether
EARL can correctly solve the question. (b): distribution of predictions
over number of tokens for EARL and SFT+GRPO.}
\label{fig:token_len}
\end{figure}

==> resources/tables/table_gsm8k.tex <==
% \begin{table}[]
% \begin{tabular}{ccccc}
% \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Category}} & \multicolumn{2}{c}{\textbf{Number of Instances}} & \multirow{2}{*}{\textbf{Acc.}} \\
%                                   &                                    & \textbf{Train}          & \textbf{Test}          &                                \\
% GSM8K                             & Original                           & 7,473                   & 1,319                  & 76.27                          \\
% \multirow{2}{*}{GSM8K\_filtered}  & Original                           & 5,317                   & 579                    & 74.09                          \\
%                                   & Rewrite                            & 5,317                   & 579                    & 31.95                         
% \end{tabular}
% \end{table}

\begin{table}[!t]
\small
\centering
\caption{
Evaluation results on GSM8K variances using GPT-4o, including the original version and rewrite version.
}
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Category}} & \multicolumn{2}{c}{\textbf{Number of Instances}} & \multirow{2}{*}{\textbf{EM}} \\
\cmidrule(lr){3-4} \cmidrule(lr){4-4}
& & \textbf{Train} & \textbf{Test} & \\
\midrule
 GSM8K                             & Original                           & 7,473                   & 1,319                  & 76.27                          \\
 \midrule
 \multirow{2}{*}{GSM8K\_filtered}  & Original                           & 5,317                   & 579                    & 74.09                          \\
                                   & Rewrite                            & 5,317                   & 579                    & 31.95                          \\
\bottomrule
\end{tabular}
}
\vspace{-0.5em}
\label{table:result_gsm8k}
\vspace{-1em}
\end{table}

